VideoForensicsHQ: Detecting High-quality Manipulated Face Videos

There are concerns that new approaches to the synthesis of high quality face videos may be misused to manipulate videos with malicious intent. The research community therefore developed methods for the detection of modified footage and assembled benchmark datasets for this task. In this paper, we examine how the performance of forgery detectors depends on the presence of artefacts that the human eye can see. We introduce a new benchmark dataset for face video forgery detection, of unprecedented quality. It allows us to demonstrate that existing detection techniques have difficulties detecting fakes that reliably fool the human eye. We thus introduce a new family of detectors that examine combinations of spatial and temporal features and outperform existing approaches both in terms of detection accuracy and generalization.

==> more_results.tex <==


We have evaluated the impact of compression on the test accuracy of all detectors on our dataset.

Our first experiments showed that applying the same compression to our data as was applied to \setff{} by \emph{R\"ossler et al.} \cite{roessler2019faceforensics++} does not lead to the expected drop in detection accuracy. 
The reason is that the face regions in our dataset (average size $488\times 488$ pixels) are much larger than in \setff (average size $258 \times 258$). Since compression happens \emph{before} we detect square face crops and resize them to the detector input resolution of $299 \times 299$, compression artifacts hurt the quality of our higher-resolution video much less than that of \emph{R\"ossler et al.} \cite{roessler2019faceforensics++}.


This is why we have resized all videos in our dataset to contain the same average face crop resolution as in \setff{} and \emph{then} compressed the result, before we applied face crop extraction. See \cref{fig:scaledcompression} for example results.  \cref{tab:compression_scaled} reports the expected decrease in detector performance: Light compression already leads to significant deterioration, with our detectors still outperforming previous methods. While $\S$, though based exclusively on high-frequency spatial information suffers least under light compression, the picture changes as the compression level is increased: $\S$ is now performing worst among our detectors, which still outperform the baselines. However, they do so by a much smaller margin and with the exception of \mesonet{}, that is now on par with the simpler ones.





\newcommand{\cframe}[1]{\includegraphics[width=2.75cm]{pics/#1.png}}
\begin{figure}

\center
\vspace{-0.5cm}
\begin{turn}{90}
\begin{tabular}{c c c c c c }

FF++  & FF++   & \DSName{} &  \DSName{} &  \DSName{} &  \DSName{} \\
real & fake & real (original) & fake (original) & real (resized) & fake (resized) \\

\cframe{000_real} & \cframe{000_fake} & \cframe{rd0_real} & \cframe{rd0_fake} & \cframe{srd0_real} & \cframe{srd0_fake} \\
\cframe{001_real} & \cframe{001_fake} & \cframe{rd1_real} & \cframe{rd1_fake} & \cframe{srd1_real} & \cframe{srd1_fake} \\
\cframe{002_real} & \cframe{002_fake} & \cframe{yt0_real} & \cframe{yt0_fake} & \cframe{syt0_real} & \cframe{syt0_fake} \\
\cframe{005_real} & \cframe{005_fake} & \cframe{sa1_real} & \cframe{sa1_fake} & \cframe{ssa1_real} & \cframe{ssa1_fake} \\
\end{tabular}
\end{turn}
\caption{A comparison of reals and fakes, all resulting from H.264 compression with constant rate factor 40, and then preprocessed as input to the detectors. If the \DSName{} videos are not resized before they are compressed, compression has much less impact on video quality and thus detection accuracy. These examples are better viewed on screen than on paper.}
\label{fig:scaledcompression}
\end{figure}



\begin{table}
\vspace{-1cm}

\center
\noindent\begin{minipage}{0.8\textwidth}
\center
\vspace{-0.5cm}
\begin{minipage}[c][6cm][c]{\dimexpr0.5\textwidth-0.5\Colsep\relax}
Light compression (CRF 23)
\vspace{5pt}



\begin{tabular}{|c|c|c|}
\hline
\arch & \valcompact & \acc{} \\
\hline
$\C$ & 63.34\%@23 & 71.16\%\\
$\S$ & 84.68\%@13 & 83.58\%\\
$\CS$ & 84.34\%@5 & 76.33\%\\
$\CST$ & 83.93\%@3 & 78.65\%\\
\mesonet & 62.34\%@3 & 68.27\%\\
\easyspot & 57.61\%@3 & 52.40\%\\
\simplelinear & 60.91\%@15 & 58.51\%\\
\misl & 76.25\%@6 & 69.99\%\\
\hline
\end{tabular}
\end{minipage}
\begin{minipage}[c][6cm][c]{\dimexpr0.5\textwidth-0.5\Colsep\relax}

Strong compression (CRF 40)

\vspace{5pt}



\begin{tabular}{|c|c|c|}
\hline
\arch & \valcompact & \acc{} \\
\hline
$\C$ & 60.41\%@12 & 64.84\%\\
$\S$ & 65.48\%@4 & 60.19\%\\
$\CS$ & 63.06\%@5 & 67.53\%\\
$\CST$ & 61.10\%@8 & 65.49\%\\
\mesonet & 56.85\%@3 & 63.89\%\\
\easyspot & 51.20\%@3 & 47.88\%\\
\simplelinear & 57.70\%@14 & 53.16\%\\
\misl & 64.31\%@5 & 57.39\%\\
\hline
\end{tabular}
\end{minipage}%
\end{minipage}

\vspace{-0.5cm}
\caption{Validation maxima and test accuracies of all evaluated detectors, trained on the same H.264 compression levels as in \emph{R\"ossler et al.} \cite{roessler2019faceforensics++}, i.e. \enquote{light compression} (constant rate factor 23) and \enquote{strong compression} (constant rate factor 40). Training was stopped if validation accuracy did not see a new maximum for 10 consecutive epochs. All numbers are averages of three independent training runs. Since the videos in our dataset are of much higher resolution than in \setff{}, and since in addition the face regions are much larger relative to the video resolution, we have resized all our videos such that the average face crop resolution in each video over time is equal to the one found in \setff{}. Only after that we applied compression and then preprocessed the result as input for the evaluated detectors.}
\label{tab:compression_scaled}
\vspace{-0.75cm}
\end{table}



